Think Before You Act: Decision Gate for LLM Agents

LLM agents increasingly perform consequential actions through external tools, yet their proposed actions are often executed without independent verification of policy compliance or task completion. We introduce JevAct, a runtime verification framework that intercepts selected agent actions before execution and enables feedback-driven correction. JevAct compiles domain policies into executable state checks and structured questions evaluated by a prefill-only decision model, which produces probability-based judgments without relying on LLM generation. By combining deterministic verification of tool-state facts with probabilistic assessment of conversational context, the framework identifies potentially invalid actions and premature task termination, providing targeted feedback for bounded revision. JevAct operates independently of the underlying agent model and requires no modifications to its parameters or tools. We evaluate JevAct across eleven LLM agents on $\tau^2$-bench Airline and Telecom tasks and BFCL. Results show improvements in agent reliability across multiple models and benchmarks, with particularly consistent gains on Telecom and BFCL, while performance on Airline is more mixed. Overall, these findings suggest that combining structured decision models with executable verification can improve the reliability of tool-using LLM agents.

==> tables/judge_inputs.tex <==
% generated by scripts/make_tables.py -- do not edit by hand
\begin{tabular}{@{}l r r r r@{}}
\toprule
Check (Kev-27B runs, seeds 400--402) & Checks & Median & 90th pct. & Over 8,192 \\
\midrule
Airline write gate & 528 & 7,342 & 14,654 & 41\% \\
Telecom hand-off check & 1,595 & 4,032 & 7,056 & 4\% \\
\midrule
Airline write gate, flagged by Kev's questions & \multicolumn{2}{r}{input $\le$ 8,192} & \multicolumn{2}{r}{input $>$ 8,192} \\
\midrule
Kev-27B & \multicolumn{2}{r}{59/310 (19\%)} & \multicolumn{2}{r}{39/218 (18\%)} \\
Kev-9B & \multicolumn{2}{r}{19/316 (6\%)} & \multicolumn{2}{r}{5/168 (3\%)} \\
Kev-0.8B & \multicolumn{2}{r}{0/332 (0\%)} & \multicolumn{2}{r}{0/172 (0\%)} \\
\bottomrule
\end{tabular}


==> tables/offline_judges.tex <==
% generated by scripts/make_tables.py -- do not edit by hand
\begin{tabular}{@{}l ccc@{}}
\toprule
Judge & Kev-27B & Kev-9B & Kev-0.8B \\
\midrule
\multicolumn{4}{@{}l}{\textit{A. Same decisions as Kev-27B? (609 hand-off states)}} \\
Hand-offs flagged & 371 & 369 & 342 \\
Same flag / pass decision as Kev-27B & -- & 97.0\% & 90.6\% \\
Same steps named in the feedback & -- & 67.7\% & 37.6\% \\
\midrule
\multicolumn{4}{@{}l}{\textit{B. Catches: the fix the task needs is still undone; is it flagged? (higher is better)}} \\
Line roaming not enabled (69 states) & 56 (81\%) & 57 (83\%) & 55 (80\%) \\
Device roaming switch off (203) & 70 (34\%) & 70 (34\%) & 69 (34\%) \\
Data limit exceeded, not refueled (261) & 193 (74\%) & 189 (72\%) & 175 (67\%) \\
\midrule
\multicolumn{4}{@{}l}{\textit{C. False alarms: a fix the task does not need is flagged (lower is better)}} \\
Roaming, task has no roaming fault (71) & 56 (79\%) & 57 (80\%) & 53 (75\%) \\
Refuel, data limit not exceeded (174) & 137 (79\%) & 138 (79\%) & 117 (67\%) \\
\midrule
\multicolumn{4}{@{}l}{\textit{D. Says the problem is already fixed, which switches the check off}} \\
In episodes that ended failed (380) & 0 & 0 & 11 \\
\bottomrule
\end{tabular}


==> tables/telecom_handoff.tex <==
% generated by scripts/make_tables.py -- do not edit by hand
\begin{tabular}{@{}l cc cc@{}}
\toprule
 & \multicolumn{2}{c}{Failed after a transfer (\%)} & \multicolumn{2}{c}{Hand-off flagged (\jevact{})} \\
\cmidrule(lr){2-3} \cmidrule(l){4-5}
Model & ReAct & \jevact{} & Episodes & Solved (\%) \\
\midrule
GPT-4.1 & 50.3 & 29.2 & 209 & 37 \\
Haiku 4.5 & 53.2 & 34.2 & 217 & 34 \\
Opus 4.6 & 38.9 & 5.3 & 128 & 91 \\
Opus 5.5 & 5.0 & 3.8 & 10 & 20 \\
gpt-oss-20b & 22.2 & 9.6 & 83 & 39 \\
gpt-oss-120b & 43.0 & 19.0 & 139 & 58 \\
Qwen3.8-27B & 21.1 & 4.1 & 49 & 76 \\
DeepSeek-V4-Pro & 28.1 & 11.1 & 83 & 84 \\
\bottomrule
\end{tabular}

